Structural Knowledge Distillation for Object Detection

Knowledge Distillation (KD) is a well-known training paradigm in deep neural networks where knowledge acquired by a large teacher model is transferred to a small student. KD has proven to be an effective technique to significantly improve the student's performance for various tasks including object detection. As such, KD techniques mostly rely on guidance at the intermediate feature level, which is typically implemented by minimizing an lp-norm distance between teacher and student activations during training. In this paper, we propose a replacement for the pixel-wise independent lp-norm based on the structural similarity (SSIM). By taking into account additional contrast and structural cues, feature importance, correlation and spatial dependence in the feature space are considered in the loss formulation. Extensive experiments on MSCOCO demonstrate the effectiveness of our method across different training schemes and architectures. Our method adds only little computational overhead, is straightforward to implement and at the same time it significantly outperforms the standard lp-norms. Moreover, more complex state-of-the-art KD methods using attention-based sampling mechanisms are outperformed, including a +3.5 AP gain using a Faster R-CNN R-50 compared to a vanilla model.

==> guidelines.tex <==
\section{Submission of papers to NeurIPS 2022}


Please read the instructions below carefully and follow them faithfully.


\subsection{Style}


Papers to be submitted to NeurIPS 2022 must be prepared according to the
instructions presented here. Papers may only be up to {\bf nine} pages long,
including figures. Additional pages \emph{containing only acknowledgments and
references} are allowed. Papers that exceed the page limit will not be
reviewed, or in any other way considered for presentation at the conference.


The margins in 2022 are the same as those in 2007, which allow for $\sim$$15\%$
more words in the paper compared to earlier years.


Authors are required to use the NeurIPS \LaTeX{} style files obtainable at the
NeurIPS website as indicated below. Please make sure you use the current files
and not previous versions. Tweaking the style files may be grounds for
rejection.


\subsection{Retrieval of style files}


The style files for NeurIPS and other conference information are available on
the World Wide Web at
\begin{center}
  \url{http://www.neurips.cc/}
\end{center}
The file \verb+neurips_2022.pdf+ contains these instructions and illustrates the
various formatting requirements your NeurIPS paper must satisfy.


The only supported style file for NeurIPS 2022 is \verb+neurips_2022.sty+,
rewritten for \LaTeXe{}.  \textbf{Previous style files for \LaTeX{} 2.09,
  Microsoft Word, and RTF are no longer supported!}


The \LaTeX{} style file contains three optional arguments: \verb+final+, which
creates a camera-ready copy, \verb+preprint+, which creates a preprint for
submission to, e.g., arXiv, and \verb+nonatbib+, which will not load the
\verb+natbib+ package for you in case of package clash.


\paragraph{Preprint option}
If you wish to post a preprint of your work online, e.g., on arXiv, using the
NeurIPS style, please use the \verb+preprint+ option. This will create a
nonanonymized version of your work with the text ``Preprint. Work in progress.''
in the footer. This version may be distributed as you see fit. Please \textbf{do
  not} use the \verb+final+ option, which should \textbf{only} be used for
papers accepted to NeurIPS.


At submission time, please omit the \verb+final+ and \verb+preprint+
options. This will anonymize your submission and add line numbers to aid
review. Please do \emph{not} refer to these line numbers in your paper as they
will be removed during generation of camera-ready copies.


The file \verb+neurips_2022.tex+ may be used as a ``shell'' for writing your
paper. All you have to do is replace the author, title, abstract, and text of
the paper with your own.


The formatting instructions contained in these style files are summarized in
Sections \ref{gen_inst}, \ref{headings}, and \ref{others} below.


\section{General formatting instructions}
\label{gen_inst}


The text must be confined within a rectangle 5.5~inches (33~picas) wide and
9~inches (54~picas) long. The left margin is 1.5~inch (9~picas).  Use 10~point
type with a vertical spacing (leading) of 11~points.  Times New Roman is the
preferred typeface throughout, and will be selected for you by default.
Paragraphs are separated by \nicefrac{1}{2}~line space (5.5 points), with no
indentation.


The paper title should be 17~point, initial caps/lower case, bold, centered
between two horizontal rules. The top rule should be 4~points thick and the
bottom rule should be 1~point thick. Allow \nicefrac{1}{4}~inch space above and
below the title to rules. All pages should start at 1~inch (6~picas) from the
top of the page.


For the final version, authors' names are set in boldface, and each name is
centered above the corresponding address. The lead author's name is to be listed
first (left-most), and the co-authors' names (if different address) are set to
follow. If there is only one co-author, list both author and co-author side by
side.


Please pay special attention to the instructions in Section \ref{others}
regarding figures, tables, acknowledgments, and references.


\section{Headings: first level}
\label{headings}


All headings should be lower case (except for first word and proper nouns),
flush left, and bold.


First-level headings should be in 12-point type.


\subsection{Headings: second level}


Second-level headings should be in 10-point type.


\subsubsection{Headings: third level}


Third-level headings should be in 10-point type.


\paragraph{Paragraphs}


There is also a \verb+\paragraph+ command available, which sets the heading in
bold, flush left, and inline with the text, with the heading followed by 1\,em
of space.


\section{Citations, figures, tables, references}
\label{others}


These instructions apply to everyone.


\subsection{Citations within the text}


The \verb+natbib+ package will be loaded for you by default.  Citations may be
author/year or numeric, as long as you maintain internal consistency.  As to the
format of the references themselves, any style is acceptable as long as it is
used consistently.


The documentation for \verb+natbib+ may be found at
\begin{center}
  \url{http://mirrors.ctan.org/macros/latex/contrib/natbib/natnotes.pdf}
\end{center}
Of note is the command \verb+\citet+, which produces citations appropriate for
use in inline text.  For example,
\begin{verbatim}
   \citet{hasselmo} investigated\dots
\end{verbatim}
produces
\begin{quote}
  Hasselmo, et al.\ (1995) investigated\dots
\end{quote}


If you wish to load the \verb+natbib+ package with options, you may add the
following before loading the \verb+neurips_2022+ package:
\begin{verbatim}
   \PassOptionsToPackage{options}{natbib}
\end{verbatim}


If \verb+natbib+ clashes with another package you load, you can add the optional
argument \verb+nonatbib+ when loading the style file:
\begin{verbatim}
   \usepackage[nonatbib]{neurips_2022}
\end{verbatim}


As submission is double blind, refer to your own published work in the third
person. That is, use ``In the previous work of Jones et al.\ [4],'' not ``In our
previous work [4].'' If you cite your other papers that are not widely available
(e.g., a journal paper under review), use anonymous author names in the
citation, e.g., an author of the form ``A.\ Anonymous.''


\subsection{Footnotes}


Footnotes should be used sparingly.  If you do require a footnote, indicate
footnotes with a number\footnote{Sample of the first footnote.} in the
text. Place the footnotes at the bottom of the page on which they appear.
Precede the footnote with a horizontal rule of 2~inches (12~picas).


Note that footnotes are properly typeset \emph{after} punctuation
marks.\footnote{As in this example.}


\subsection{Figures}


\begin{figure}
  \centering
  \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
  \caption{Sample figure caption.}
\end{figure}


All artwork must be neat, clean, and legible. Lines should be dark enough for
purposes of reproduction. The figure number and caption always appear after the
figure. Place one line space before the figure caption and one line space after
the figure. The figure caption should be lower case (except for first word and
proper nouns); figures are numbered consecutively.


You may use color figures.  However, it is best for the figure captions and the
paper body to be legible if the paper is printed in either black/white or in
color.


\subsection{Tables}


All tables must be centered, neat, clean and legible.  The table number and
title always appear before the table.  See Table~\ref{sample-table}.


Place one line space before the table title, one line space after the
table title, and one line space after the table. The table title must
be lower case (except for first word and proper nouns); tables are
numbered consecutively.


Note that publication-quality tables \emph{do not contain vertical rules.} We
strongly suggest the use of the \verb+booktabs+ package, which allows for
typesetting high-quality, professional tables:
\begin{center}
  \url{https://www.ctan.org/pkg/booktabs}
\end{center}
This package was used to typeset Table~\ref{sample-table}.


\begin{table}
  \caption{Sample table title}
  \label{sample-table}
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Part}                   \\
    \cmidrule(r){1-2}
    Name     & Description     & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal  & $\sim$100     \\
    Axon     & Output terminal & $\sim$10      \\
    Soma     & Cell body       & up to $10^6$  \\
    \bottomrule
  \end{tabular}
\end{table}


\section{Final instructions}


Do not change any aspects of the formatting parameters in the style files.  In
particular, do not modify the width or length of the rectangle the text should
fit into, and do not change font sizes (except perhaps in the
\textbf{References} section; see below). Please note that pages should be
numbered.


\section{Preparing PDF files}


Please prepare submission files with paper size ``US Letter,'' and not, for
example, ``A4.''


Fonts were the main cause of problems in the past years. Your PDF file must only
contain Type 1 or Embedded TrueType fonts. Here are a few instructions to
achieve this.


\begin{itemize}


\item You should directly generate PDF files using \verb+pdflatex+.


\item You can check which fonts a PDF files uses.  In Acrobat Reader, select the
  menu Files$>$Document Properties$>$Fonts and select Show All Fonts. You can
  also use the program \verb+pdffonts+ which comes with \verb+xpdf+ and is
  available out-of-the-box on most Linux machines.


\item The IEEE has recommendations for generating PDF files whose fonts are also
  acceptable for NeurIPS. Please see
  \url{http://www.emfield.org/icuwb2010/downloads/IEEE-PDF-SpecV32.pdf}


\item \verb+xfig+ "patterned" shapes are implemented with bitmap fonts.  Use
  "solid" shapes instead.


\item The \verb+\bbold+ package almost always uses bitmap fonts.  You should use
  the equivalent AMS Fonts:
\begin{verbatim}
   \usepackage{amsfonts}
\end{verbatim}
followed by, e.g., \verb+\mathbb{R}+, \verb+\mathbb{N}+, or \verb+\mathbb{C}+
for $\mathbb{R}$, $\mathbb{N}$ or $\mathbb{C}$.  You can also use the following
workaround for reals, natural and complex:
\begin{verbatim}
   \newcommand{\RR}{I\!\!R} %real numbers
   \newcommand{\Nat}{I\!\!N} %natural numbers
   \newcommand{\CC}{I\!\!\!\!C} %complex numbers
\end{verbatim}
Note that \verb+amsfonts+ is automatically loaded by the \verb+amssymb+ package.


\end{itemize}


If your file contains type 3 fonts or non embedded TrueType fonts, we will ask
you to fix it.


\subsection{Margins in \LaTeX{}}


Most of the margin problems come from figures positioned by hand using
\verb+\special+ or other commands. We suggest using the command
\verb+\includegraphics+ from the \verb+graphicx+ package. Always specify the
figure width as a multiple of the line width as in the example below:
\begin{verbatim}
   \usepackage[pdftex]{graphicx} ...
   \includegraphics[width=0.8\linewidth]{myfile.pdf}
\end{verbatim}
See Section 4.4 in the graphics bundle documentation
(\url{http://mirrors.ctan.org/macros/latex/required/graphics/grfguide.pdf})


A number of width problems arise when \LaTeX{} cannot properly hyphenate a
line. Please give LaTeX hyphenation hints using the \verb+\-+ command when
necessary.


\begin{ack}
Use unnumbered first level headings for the acknowledgments. All acknowledgments
go at the end of the paper before the list of references. Moreover, you are required to declare
funding (financial activities supporting the submitted work) and competing interests (related financial activities outside the submitted work).
More information about this disclosure can be found at: \url{https://neurips.cc/Conferences/2022/PaperInformation/FundingDisclosure}.


Do {\bf not} include this section in the anonymized submission, only in the final paper. You can use the \texttt{ack} environment provided in the style file to autmoatically hide this section in the anonymized submission.
\end{ack}

==> sections/discussion.tex <==
\section{Discussion}
% Three assumptions
% We start off this section with discussing how this work tackles each drawback of the $\ell_p$-norm, and the resulting impact on model performance. 
% First of all, spatial relationships are captured by distilling over a local area instead of individual pixels. As can be seen in row 5-8 of \cref{tab:maintable}, directly comparing these local properties does not gain a lot of performance over conventional $\ell_p$-norm. A drawback of using a local area is the loss of detail through the application of the kernel, which may cause limited performance improvement in itself. Second, spatial feature importance (i.e. which area should be distilled more) is inherently assigned by the relative comparison of the second-order properties. A difference in the lower ranges of these properties is weighted more heavily than in higher regions (see \cref{sec:trajec}), and including this relative comparison actually is key to performance as can be seen in \cref{tab:maintable}. Finally the relationship between feature spaces can be seen as the most important property. Not only does it boost performance the most, but it can also be seen in \cref{fig:comp2} it has significantly more influence on where in the feature space the loss is assigned.  

% challenge direction of research space
% One of the main objectives of this work is to furthermore challenge the direction the \acrshort{kd} detection research space has evolved in. Our qualitative experimental data (\cref{fig:focus}) suggests that the notion adopted by previous work that object regions are "knowledge-dense" is only partly true: yes they are important, but not the only thing that should be focused on. \cite{guo2021distilling} already did suggest that background information can be important in distillation, but we go one step further and extend this notion to include only second-order knowledge dense background regions with e.g. high variation in contrast, which is retained throughout the feature space.



% Rather than focusing on second-order 

% It therefore allows further research to more easily build on top of, and 


% without the associated overhead discussed in \cref{sec:introduction}. Further improvements for \acrshort{kd} may be made using more sophisticated sampling mechanisms, but as we have shown that there is a lot of second-order knowledge hidden in the discussed properties of feature spaces, we do believe that these future  gains may not lie in solely sampling object instances.

% Contrary to that method however, our method can be easily "plugged in" to a teacher-student detector combination, does not require careful tuning and can be used as a replacement of $\ell_p$-norms in future feature-based \acrshort{kd} methods. 

\paragraph{Impact on training consumption ...}
\paragraph{Convergence faster earlier epochs, loss }

\paragraph{What does the student learn from the teacher?} As initially shown by \cite{Hinton2015a}, \acrshort{kd} remains a mechanism for regularization, which is why the student is able to outperform the teacher with our method. To gain insight into what kind of knowledge is mainly transferred from the teacher, we compare the types of errors made by the teacher to our distilled model, as shown in \cref{fig:error}, where we make the distinction between classification and localization. When removing localization, our method is pushed from 40.7 to 67.2 AP, while the teacher is pushed from 40.4 to 67.8 AP. Additionally, removing class confusions adds another 10.6 AP for the student and 10.4 AP for the teacher. So the teacher is dominated by localization errors, while for the student this has been a particular point of improvement in which it even outperforms the teacher. This is an indication that the ground truth signal providing localization supervision is more dominant than the classification, while for classification the student remains limited by the teacher. This is furthermore reflected by comparing the trajectory of the classification vs. regression loss compared to a vanilla model (\cref{fig:lcurves}), where we can observe that classification loss is relatively lower compared to the regression loss, indicating the aid from the teacher.  

\paragraph{Can SSIM be combined with sampling mechanisms?}

sampling mechanisms, counterproductive ...
at the output ..

% At $AP_{75}$ we reach 43.9, while removing localization pushes our method to .672. the teacher reaches 43.2 and without localization is pushed to 67.8.

% Next to the most strict overall $AP$, our method outperforms the teacher in the stricter localization metrics ($AP_{75}$), but if we remove classification errors the teacher performs slightly better. This indicates that distillation is dominated by classification knowledge from the teacher, while for localization the student is able to surpass performance through the ground truth stimulus. 

% This is an indication that the ground truth signal providing localization is more  

% So the error in the teacher is dominated more in localization, while in our model it is more in classification errors. This indicates that the student is limited to the teacher for the classification, while it relies on the ground truth annotations for localization. /
% One limitation of \acrshort{kd} that has to be kept in mind that there is exists no "perfect teacher". Therefore finding the "perfect" signal fidelity metric as an objective function will not directly allow for perfect students. Furthermore, 

\begin{figure}[H]
\centering
    \begin{subfigure}{.245\textwidth}
    \includegraphics[width=1\textwidth]{media/error_analysis/AUC_vanilla.png}
    \caption{Vanilla}
    \label{fig:error1}
    \end{subfigure}
    \begin{subfigure}{.245\textwidth}
    \includegraphics[width=1\textwidth]{media/error_analysis/AUC_teach.png}
    \caption{Teacher}
    \label{fig:error2}
    \end{subfigure}
    \begin{subfigure}{.245\textwidth}
    \includegraphics[width=1\textwidth]{media/error_analysis/AUC_kang.png}
    \caption{\cab{kang2021instance}}
    \label{fig:error3}
    \end{subfigure}
    \begin{subfigure}{.245\textwidth}
    \includegraphics[width=1\textwidth]{media/error_analysis/AUC_ssim.png}
    \caption{Ours}
    \label{fig:error4}
    \end{subfigure}
    \caption{Distribution of error types on \acrshort{mscoco}. Area under Curve is provided in brackets in the legend: \textbf{C75} - \acrshort{pr} at box \acrshort{iou} .75 ($AP_{75}$); \textbf{C50} - \acrshort{pr} at at box \acrshort{iou} .50 ($AP_{50}$); \textbf{Loc} - \acrshort{pr} at \acrshort{iou} .10 (localization ignored, no duplicates); \textbf{Sim} - \acrshort{pr} after removal of supercategory \acrshortpl{fp}; \textbf{Oth} - \acrshort{pr} after removal of all class confusions; \textbf{BG} - \acrshort{pr} after removal of all background \acrshortpl{fp}; \textbf{FN} - False Negative predictions ($AP = 1$).}
     \label{fig:error}
\end{figure}

\begin{figure}[h]
\centering
    \begin{subfigure}{.49\textwidth}
    \includegraphics[width=1\textwidth]{media/error_analysis/loss_curve_vanilla.png}
    \caption{Vanilla}
    \label{fig:lcurves1}
    \end{subfigure}
    \begin{subfigure}{.49\textwidth}
    \includegraphics[width=1\textwidth]{media/error_analysis/loss_curve_ssim.png}
    \caption{ssim}
    \label{fig:lcurves2}
    \end{subfigure}
    \caption{loss curves}
     \label{fig:lcurves}
\end{figure}



% \paragraph{What is the effect of sampling objects?}
% One of the main objectives of this work has been to challenge the direction the \acrshort{kd} detection research space has evolved in, and as we observe that our performance is on par with current state-of-the-art \cite{kang2021instance, zhang2020improve}, we argue that we have achieved that goal. Contrary to previous work, our approach simply introduces a replacement for $\ell_p$-norms in future feature-based \acrshort{kd} methods, which without any sophisticated sampling mechanisms achieves comparable performance. We have furthermore demonstrated that there is a lot of knowledge present in the statistical properties of feature spaces, in particular in cross-correlation. 

% We therefore believe that there might be more potential gains to be made in the \acrshort{kd} domain by finding ways to further exploit this second-order knowledge rather than by solely focusing on sampling object instances.

==> sections/discussion2.tex <==
\section{Understanding the Importance of Statistical Properties} \label{sec:discussion}
% In the previous section we provided the quantitative results of adopting $\ell_{\text{SSIM}}$ as an objective function in distillation, where it could be observed that 
The central value proposition of implementing $\ell_{\text{SSIM}}$ over an $\ell_{p}$-norm as an objective function is that it is able to extract knowledge manifested in three strong statistical properties of the feature space, recall \cref{sec:relatedwork}: (i) the unequal importance of features, (ii) the spatial dependency between features, and (iii) the dependency between the teacher and student feature space. In this section we first analyze the gradient distribution of the feature space for $\ell_{\text{SSIM}}$  and for the $\ell_{p}$-norm, and additionally for each component $l$, $c$, $s$ in $\ell_{\text{SSIM}}$. This allows us to, combined with the quantitative results in the previous section, gain insight as to what the impact is of leveraging each of the three feature space properties. 

% and the distribution of the loss depending on the area in order to discuss how important each of these properties is for distillation. 

\subsection{Gradient Analysis} \label{sec:distr}
% \begin{figure}[h]
% \centering
% % Waveform
% \begin{subfigure}[b]{0.166\textwidth}
% \includegraphics[width =\textwidth]{media/fmap_comparison/beach.jpg}
% \label{fig:tc}\vspace{-1.12\baselineskip}
% \includegraphics[width =\textwidth]{media/discussion/img.png}
% \label{fig:tc}\vspace{-1.12\baselineskip}
% \includegraphics[width =\textwidth]{media/fmap_comparison/livingroom.jpg}
% \label{fig:tc}\vspace{-1.12\baselineskip}
% \includegraphics[width =\textwidth]{media/fmap_comparison/zebra.jpg}\caption{Image}\label{fig:focus0}
% \end{subfigure}%
% \begin{subfigure}[b]{0.166\textwidth}
% \includegraphics[width =\textwidth]{media/fmap_comparison/all_beach/beach_mean_teacher_norm.png}
% \label{fig:tc}\vspace{-1.12\baselineskip}
% \includegraphics[width =\textwidth]{media/fmap_comparison/car_mean_teacher_norm.png}
% \label{fig:tc}\vspace{-1.12\baselineskip}
% \includegraphics[width =\textwidth]{media/fmap_comparison/lr_mean_teacher_norm.png}
% \label{fig:tc}\vspace{-1.12\baselineskip}
% \includegraphics[width =\textwidth]{media/fmap_comparison/zebra_mean_teacher_norm.png}\caption{Teacher}\label{fig:focus1}
% \end{subfigure}%
% \begin{subfigure}[b]{0.166\textwidth}
% \includegraphics[width =\textwidth]{media/fmap_comparison/all_beach/beach_mean_student_norm.png}
% \label{fig:tc}\vspace{-1.12\baselineskip}
% \includegraphics[width =\textwidth]{media/fmap_comparison/car_mean_student_norm.png}
% \label{fig:tc}\vspace{-1.12\baselineskip}
% \includegraphics[width =\textwidth]{media/fmap_comparison/lr_mean_student_norm.png}
% \label{fig:tc}\vspace{-1.12\baselineskip}
% \includegraphics[width =\textwidth]{media/fmap_comparison/zebra_mean_student_norm.png}\caption{Student}\label{fig:focus2}
% \end{subfigure}%
% \begin{subfigure}[b]{0.166\textwidth}
% \includegraphics[width =\textwidth]{media/fmap_comparison/all_beach/beach_mean_l1_norm.png}
% \label{fig:tc}\vspace{-1.12\baselineskip}
% \includegraphics[width =\textwidth]{media/fmap_comparison/car_mean_l1_norm.png}
% \label{fig:tc}\vspace{-1.12\baselineskip}
% \includegraphics[width =\textwidth]{media/fmap_comparison/lr_mean_l1_norm.png}
% \label{fig:tc}\vspace{-1.12\baselineskip}
% \includegraphics[width =\textwidth]{media/fmap_comparison/zebra_mean_l1_norm.png}\caption{$\ell_1$-norm}\label{fig:focus4}
% \end{subfigure}%
% \begin{subfigure}[b]{0.166\textwidth}
% \includegraphics[width =\textwidth]{media/fmap_comparison/all_beach/beach_mean_l2_norm.png}
% \label{fig:tc}\vspace{-1.12\baselineskip}
% \includegraphics[width =\textwidth]{media/fmap_comparison/car_mean_l2_norm.png}
% \label{fig:tc}\vspace{-1.12\baselineskip}
% \includegraphics[width =\textwidth]{media/fmap_comparison/lr_mean_l2_norm.png}
% \label{fig:tc}\vspace{-1.12\baselineskip}
% \includegraphics[width =\textwidth]{media/fmap_comparison/zebra_mean_l2_norm.png}\caption{$\ell_2$-norm}\label{fig:focus5}
% \end{subfigure}%
% \begin{subfigure}[b]{0.166\textwidth}
% \includegraphics[width =\textwidth]{media/fmap_comparison/all_beach/beach_mean_ssim_norm.png}
% \label{fig:tc}\vspace{-1.12\baselineskip}
% \includegraphics[width =\textwidth]{media/fmap_comparison/car_mean_ssim_norm.png}
% \label{fig:tc}\vspace{-1.12\baselineskip}
% \includegraphics[width =\textwidth]{media/fmap_comparison/lr_mean_ssim_norm.png}
% \label{fig:tc}\vspace{-1.12\baselineskip}
% \includegraphics[width =\textwidth]{media/fmap_comparison/zebra_mean_ssim_norm.png}\caption{$\ell_{\text{ssim}}$}\label{fig:focus3}
% \end{subfigure}%
% \caption{Aggregated mean feature map distributions. (b), (c) denote teacher and student feature maps.  All feature maps are normalized [0,1].}\label{fig:focus}
% \end{figure}



% In \cref{fig:focus} we provide examples of how the training stimulus is distributed in the feature space, dependent on which training objective is used. \Cref{fig:focus1}, \ref{fig:focus2} demonstrate the aggregated mean feature map intensities ($r=1$) of a freshly initialized RetinaNet-R50 student and fully trained R101 teacher \cite{lin2017focal} respectively. In \cref{fig:focus3} it can be observed that with $\ell_{\text{ssim}}$, particular importance is given to regions where there is a distinct difference in contrast, such as a transition from ground to sky, and in general to silhouettes of clearly isolated objects. Furthermore it can be observed that very little importance is given to low-contrast background regions, while more diverse background regions are targeted. In \cref{fig:focus3} the gradient distribution for the $\ell_p$-norm ($p=2$) can be observed. It can be noticed that certain edges of objects are mainly targeted, and additionally relatively bright areas such as the window or the sky. 



% Furthermore, $\ell_1$ provides a more distributed allocation of the loss than $\ell_2$.

% \begin{figure}[H]
% \centering
%     \begin{subfigure}{0.325\textwidth}
%     \includegraphics[width=1.0\textwidth]{media/discussion/img.png}
%     \caption{Input Image}
%     \label{fig:focusimg}
%     \end{subfigure}
%     \begin{subfigure}{0.325\textwidth}
%     \includegraphics[width=1\textwidth]{media/discussion/mean_student_norm.png}
%     \caption{Student}
%     \label{fig:focus0}
%     \end{subfigure}
%     \begin{subfigure}{0.325\textwidth}
%     \includegraphics[width=1\textwidth]{media/discussion/mean_teacher_norm.png}
%     \caption{Teacher}
%     \label{fig:focus1}
%     \end{subfigure} 
%     \begin{subfigure}{0.325\textwidth}
%     \includegraphics[width=1\textwidth]{media/discussion/mean_l1_norm.png}
%     \caption{$\ell_1$-norm}
%     \label{fig:focus2}
%     \end{subfigure} 
%     \begin{subfigure}{0.325\textwidth}
%     \includegraphics[width=1\textwidth]{media/discussion/mean_l2_norm.png}
%     \caption{$\ell_2$-norm}
%     \label{fig:focus3}
%     \end{subfigure} 
%     \begin{subfigure}{0.325\textwidth}
%     \includegraphics[width=1\textwidth]{media/discussion/mean_ssim_norm.png}
%     \caption{$\ell_{\text{ssim}}$}
%     \label{fig:focus4}
%     \end{subfigure} 
%     \caption{(b), (c) Aggregated mean feature maps. (d), (e), (f) Respective aggregated mean error maps. Normalized [0,1]. }
%     \label{fig:focus}
% \end{figure}

 
% \begin{figure}[h]
% \centering
%     \begin{subfigure}{.24\textwidth}
%     \includegraphics[width=1\textwidth]{media/discussion/base.png}
%     \caption{fmaps}
%     \label{fig:comp0}
%     \end{subfigure}
%     \begin{subfigure}{.24\textwidth}
%     \includegraphics[width=1\textwidth]{media/discussion/lum.png}
%     \caption{Mean Comparison}
%     \label{fig:comp1}
%     \end{subfigure} 
%     \begin{subfigure}{.24\textwidth}
%     \includegraphics[width=1\textwidth]{media/discussion/con.png}
%     \caption{Contrast}
%     \label{fig:comp2}
%     \end{subfigure}
%     \begin{subfigure}{.24\textwidth}
%     \includegraphics[width=1\textwidth]{media/discussion/str.png}
%     \caption{Correlation}
%     \label{fig:comp3}
%     \end{subfigure}
%     \label{fig:comp}
%     \caption{Comparison of feature map loss assignment}
% \end{figure}

\subsection{What is the Impact of Leveraging Each Statistical Property?}
\paragraph{Relationship between Teacher and Student} This property is captured by the structure comparison, or cross-correlation, between the feature spaces. Our prime observation is that capturing this property is the most important when it comes to improving \acrshort{kd} performance, not only because it boosts performance more compared to other components (\cref{tab:maintable}), but it can also be seen in \cref{fig:comp2} that it has significantly more influence on where in the feature space the loss is assigned. Adding luminance and contrast comparisons does however improve performance even further, indicating that structure is not mutually exclusive to other distillation objectives.   

\paragraph{Feature Importance}
Spatial feature importance has been the main property targeted by previous work through the design of object sampling mechanisms \cite{Li2017, wang2019distilling, dai2021general, zhixing2021distilling, kang2021instance}. Our qualitative experimental data suggests that this notion that object regions are "knowledge-dense" is only partly true. In \cref{fig:focus5} it can be seen that for $\ell_{\text{ssim}}$ object regions do have high gradients, but that background regions with e.g. high variation in contrast also have high gradients. Furthermore, in \cref{fig:comp3} it can be observed that structure, which has the highest impact on the loss, also posesses particularly high gradients in both object as well as high contrast background regions. Finally, feature importance is assigned relatively through $l$ and $c$, which is illustrated in \cref{fig:comp1}, \ref{fig:comp2}, where regions are assigned higher gradients based on their relative differences in $\mu$ and $\sigma$ respectively. This notion is furthermore reflected in a comparison of row 5,6 to 7,8 of \cref{tab:maintable}, where direct comparisons of $\mu$ and $\sigma$ are outperformed by relative comparisons. All taken into account, \cite{guo2021distilling} already did suggest that background information can be important in distillation, but we extend this notion to include only second-order knowledge dense background regions with e.g. high variation in contrast and low cross-correlation.

\paragraph{Spatial Relationships Between Features}
Spatial relationships are captured by distilling over a local area instead of individual pixels, which we achieve by applying a (Gaussian) kernel. This has the consequence that we trade off detail for noise reduction. Directly distilling such a "smoothed" feature map (\cref{fig:comp1}) does not result in significant performance gain over conventional $\ell_p$-norms, as can be observed in row 5,7 of \cref{tab:maintable}. This tells us that retaining detail contained in feature maps is an important factor. Where previous work implicitly retained this detail, in our method it is retained in the normalized feature maps, as can be seen in \cref{fig:comp4}.

% $c$ does target significantly distinctive areas compared to structure, and including it as a distillation driver does significantly improve 

% It is however essential to conduct the direct structure comparison, and when added together results in slightly better performance, as can be seen in row 8-11 of \cref{tab:maintable}. 

% implies making a trade-off between less noise, but also less detail.

% As can be seen in row 5-8 of \cref{tab:maintable}, solely comparing these local properties does not gain . Two things stand out here: first,  

% A drawback of using a local area is that it trades off detail in pure loss of detail through the application of the kernel as can be observed, which may cause limited performance improvement in itself. 



% not the only thing that is put importance on. \cite{guo2021distilling} already did suggest that background information can be important in distillation, but we go one step further and extend this notion to include only second-order knowledge dense background regions with e.g. high variation in contrast, which is retained throughout the feature space. It can be furthermore concluded from row 5,6 to 7,8 of \cref{tab:maintable} that this relative importance is 




% and including this relative comparison actually is key to performance as can be seen in \cref{tab:maintable}.

% is inherently assigned by the relative comparison of the second-order properties. A difference in the lower ranges of these properties is weighted more heavily than in higher regions (see \cref{sec:trajec}), 











% Finally, as \cite{kang2021instance} use attention to transform features into a subspace where spatial relation of the feature maps is not retained, therefore ssim does not work. Future work can go into improving sampling methods, but we open up a new direction which 


% Architecturally our method compares to \cite{zhang2020improve}, who use non-local modules to capture relational information between features, however it is not evident how it works and our results are better. 



% As lssim does not require labeled data future work can include application on additional tasks.







%%% GRAVEYARD %%%

% It is noteworthy that we can compete with state-of-the-art methods in this domain with a method that is very straightforward to implement. 


% Recall that 

% % What is actually important in Distillation?



% which indicates that cross-correlation the most fundamental property in this method.

% TACKLE EACH ASSUMPTION:
% \\
% 1. FEATURE INDEPENDENCE - DEMONSTRATE THAT FMAPS HAVE SPATIAL RELATIONSHIPS
% \\
% 2. EQUAL IMPORTANCE - SHOW WHAT AREAS SSIM FOCUSES ON. SHOW WHAT AREAS EACH PROPERTY FOCUSES ON
% \\
% 3. INDEPENDENCE BETWEEN FMAPS - CORRELATION ...

% In this section our aim is to provide statistical evidence of how our approach provides solutions to each of the assumptions made with existing methods, and why leverigang second-order knowledge improves distillation. Starting in \cref{sec:sd}, we demonstrate why it cannot be implicitly assumed that the features are statistically independent in the spatial dimension, and capturing second-order properties contains additional knowledge. In \cref{sec:featimp} we demonstrate how extracting and comparing second-order properties inherently assigns importance to regions, and finally in \cref{sec:rela} we analyze the impact of the relationship between $\mathcal{T}$ and $\mathcal{S}$.





==> sections/tables.tex <==
% \begin{table}[!hbt]
%     \centering
%     \begin{tabular}{l|l|lcccccc}
%     \toprule
%          Backbone & $\mathcal{L}_{\varepsilon}$ & AP & AP_{50} & AP_{75} & AP_{S} & AP_{M} & AP_{L} \\ \midrule
%          \multicolumn{8}{c}{RetinaNet [5]} \\ \midrule
%          Teacher R101  & ~ & 41.0 & 60.3 & 44.0 & 24.1 & 45.3 & 53.8 \\ 
%          \textit{Vanilla R50}  & ~ & \textit{36.4} & \textit{55.6} & \textit{38.7} & \textit{21.1} & \textit{40.3} & \textit{46.6} \\ 
%          R50 & $\ell_2$ & 36.8 (+0.4) & 55.7 & 39.1 & 20.6 & 40.5 & 47.3 \\
%          R50 & $\ell_1$ & 38.7 (+2.3) & 57.6 & 41.6 & 22.7 & 42.7 & 50.5 \\ 
%          \textbf{R50} & $\boldsymbol{\ell_{\text{SSIM}}}$ & \textbf{40.1 (+3.7)} & \textbf{59.2} & \textbf{43.1} & \textbf{23.1} & \textbf{44.6} & \textbf{53.2} \\ \midrule[0.7]
%          \multicolumn{8}{c}{ Faster R-CNN [6] } \\ \midrule
%          Teacher X101  & & 45.6 & 64.1 & 49.7 & 26.2 & 49.6 & 60.0 \\
%          \textit{Vanilla R50} & & \textit{37.4 }& \textit{58.1} & \textit{40.4} & \textit{21.2} & \textit{41.0}& \textit{48.1}  \\
%          R50  & $\ell_2$ & 37.4 (+0.0) & 57.6 & 40.9 & 21.2 & 41.3 & 48.1 \\
%          R50  & $\ell_1$ & 38.6 (+1.2) & 58.8 & 42.1 & 21.8 & 42.1 & 49.9 \\
%         \textbf{R-50} & $\boldsymbol{\ell_{\text{SSIM}}}$ & \textbf{40.9 (+3.5)} & \textbf{61.0} & \textbf{44.9} & \textbf{23.7} & \textbf{44.5} & \textbf{53.5} \\
         
%      \bottomrule
% \end{tabular}
% \label{tab:maintable}
% \end{table}

% \begin{table}
%     \centering

%     \begin{threeparttable}
%     \begin{tabular}{l|lccc|lccc}
%     \toprule
%          \multirow{2}{*}{Method}  & \multicolumn{4}{c}{RetinaNet [5]} & \multicolumn{4}{c}{Faster R-CNN [6]} \\ 
%          & AP &  AP_{S} & AP_{M} & AP_{L} & AP &  AP_{S} & AP_{M} & AP_{L} \\ \midrule
%         Teacher &  41.0 & 24.1 & 45.3 & 53.8 & 45.6 & 26.2 & 49.6 & 60.0 \\ 
          
%          \textit{Vanilla}   & \textit{36.4} & \textit{21.1} & \textit{40.3} & \textit{46.6} &  \textit{37.4} & \textit{21.2} & \textit{41.0} & \textit{48.1}\\
%          Zhang et al. [3]  & 38.5 (+2.1) & 21.7 & 42.6 & 51.5 & 38.9 (+1.5) & 21.9 & 42.1 & 51.5  \\ 
%           \textbf{Ours}   & \textbf{40.1 (+3.7)} & \textbf{23.1} & \textbf{44.6} & \textbf{53.2} & \textbf{40.9 (+3.5)}  & \textbf{23.7} & \textbf{44.5} & \textbf{53.5}  \\ \midrule
%          Teacher  & 40.4 & 24.0 & 44.3 & 52.2 & 42.0 & 25.2 & 45.6 & 54.6  \\
%          \textit{Vanilla}    & \textit{37.4} & \textit{23.1} & \textit{41.6} & \textit{48.3} &\textit{37.9} & \textit{22.4} & \textit{41.1} & \textit{49.1} \\ 
%         Kang et al.[2] \dagger & \textbf{40.7 (+3.3)} & \textbf{24.6} & 44.9 & 52.4 & 40.9 (+3.0) & \textbf{24.5} & 44.2 & 53.3 \\
%          \textbf{Ours}  \dagger & \textbf{40.7 (+3.3)} & 24.0 & \textbf{45.0} & \textbf{53.1} & \textbf{41.0 (+3.1)} & 23.8 & \textbf{44.5} & \textbf{53.7} \\
%          % CM-R-CNN X-101-FPN \cite{cai2019cascade} (Teacher) & ~ & 45.6 & 64.1 & 49.7 & 26.2 & 49.6 & 60.0 \\
%         % Faster R-CNN-R50 \cite{Ren2015} (Vanilla) & ~ & 37.4 & 58.1 & 40.4 & 21.2 & 41.0 & 48.1 \\
%         % Faster R-CNN-R50 \cite{Ren2015} (\citeauthor{zhang2020improve}) & ~ & 38.9 (+1.5) & 59.0 & 42.4 & 21.9 & 42.1 & 51.5 \\
%         % \textbf{Faster R-CNN-R50 \cite{Ren2015} (Ours)} & ~ & \textbf{40.9 (+3.5)} & \textbf{61.0} & \textbf{44.9} & \textbf{23.7} & \textbf{44.5} & \textbf{53.5} \\
         
%      \bottomrule
% \end{tabular}
% \label{tab:results_sota1}
% \end{threeparttable}
% \end{table}

% \begin{Verbatim}[commandchars=\\\{\}, frame=lines, label=l2 implementation, framesep=2mm]
% from torch.nn.functional import mse_loss
% def kd_loss(student_feats, teacher_feats):
%     \textcolor{gray}{# inputs have shape [B, C, H, W]}
%     kd_feat_loss = \textcolor{red}{mse_loss}(student_feats, teacher_feats)
%     return kd_feat_loss 
% \end{Verbatim}

% \begin{Verbatim}[commandchars=\\\{\}, frame=lines, label=ssim implementation, framesep=2mm]
% from kornia.losses import ssim_loss
% def kd_loss(student_feats, teacher_feats):
%     \textcolor{gray}{# inputs have shape [B, C, H, W]}
%     kd_feat_loss = \textcolor{blue}{ssim_loss}(student_feats, teacher_feats, \textcolor{blue}{\textcolor{blue}{window_size=11}})
%     return kd_feat_loss 
% \end{Verbatim}


\begin{equation}
    \mathcal{L}_{feat} =\sum_{r=1}^{R} \frac{1}{N_r} \sum_{h=1}^{H} \sum_{w=1}^{W} \sum_{c=1}^{C} \mathcal{L}_{\varepsilon}\bigl(\nu\left(\phi\left(\mathcal{S}_{r, h, w, c}\right)\right), \underbrace{\nu\left(\mathcal{T}_{r, h, w, c}\right)}_{\text{teacher activations}}\bigr)
\end{equation}

